Simultaneous execution of quantum circuits on current and near-future NISQ systems

In the NISQ era, multi-programming of quantum circuits (QC) helps to improve the throughput of quantum computation. Although the crosstalk, which is a major source of noise on NISQ processors, may cause performance degradation of concurrent execution of multiple QCs, its characterization cost grows quadratically in processor size. To address these challenges, we introduce palloq (parallel allocation of QCs) for improving the performance of quantum multi-programming on NISQ processors while paying attention to the combination of QCs in parallel execution and their layout on the quantum processor, and reducing unwanted interference between QCs caused by crosstalk. We also propose a software-based crosstalk detection protocol that efficiently and successfully characterizes the hardware's suitability for multi-programming. We found a trade-off between the success rate and execution time of the multi-programming. This would be attractive not only to quantum computer service but also to users around the world who want to run algorithms of suitable scale on NISQ processors that have recently attracted great attention and are being enthusiastically investigated.

==> biography.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/yohkura.png}}]{Yasuhiro Ohkura} received the B.S. degree in Policy Management from Keio University, Kanagawa, Japan in 2021.
He is currently pursuing the M.S. degree in Media and Governance at Keio University, Kanagawa, Japan.

His research interests include development of NISQ algorithm and post-NISQ computing, design the compiler for quantum computation, and Quantum Error Mitigation.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/tsatoh.png}}]{Takahiko Satoh} is a project assistant professor of Keio University Quantum Computing Center. He studied at Keio University and the University of Tokyo in 2015. He received a PhD in computer science from UT. His research field is quantum computing and quantum networking, particularly quantum network coding, NISQ algorithm design, and Quantum Internet security. He is a member of the Physical Society of Japan (JPS).
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/rdv.png}}]{Third C. Author, Jr.} (M'87) received the B.S. degree in mechanical 
engineering from National Chung Cheng University, Chiayi, Taiwan, in 2004 
and the M.S. degree in mechanical engineering from National Tsing Hua 
University, Hsinchu, Taiwan, in 2006. He is currently pursuing the Ph.D. 
degree in mechanical engineering at Texas A{\&}M University, College 
Station, TX, USA.

From 2008 to 2009, he was a Research Assistant with the Institute of 
Physics, Academia Sinica, Tapei, Taiwan. His research interest includes the 
development of surface processing and biological/medical treatment 
techniques using nonthermal atmospheric pressure plasmas, fundamental study 
of plasma sources, and fabrication of micro- or nanostructured surfaces. 

Mr. Author's awards and honors include the Frew Fellowship (Australian 
Academy of Science), the I. I. Rabi Prize (APS), the European Frequency and 
Time Forum Award, the Carl Zeiss Research Award, the William F. Meggers 
Award and the Adolph Lomb Medal (OSA).
\end{IEEEbiography}
